DMTG: One-Shot Differentiable Multi-Task Grouping

We aim to address Multi-Task Learning (MTL) with a large number of tasks by Multi-Task Grouping (MTG). Given N tasks, we propose to simultaneously identify the best task groups from 2^N candidates and train the model weights simultaneously in one-shot, with the high-order task-affinity fully exploited. This is distinct from the pioneering methods which sequentially identify the groups and train the model weights, where the group identification often relies on heuristics. As a result, our method not only improves the training efficiency, but also mitigates the objective bias introduced by the sequential procedures that potentially lead to a suboptimal solution. Specifically, we formulate MTG as a fully differentiable pruning problem on an adaptive network architecture determined by an underlying Categorical distribution. To categorize N tasks into K groups (represented by K encoder branches), we initially set up KN task heads, where each branch connects to all N task heads to exploit the high-order task-affinity. Then, we gradually prune the KN heads down to N by learning a relaxed differentiable Categorical distribution, ensuring that each task is exclusively and uniquely categorized into only one branch. Extensive experiments on CelebA and Taskonomy datasets with detailed ablations show the promising performance and efficiency of our method. The codes are available at https://github.com/ethanygao/DMTG.

==> sec/0_abstract.tex <==
\begin{abstract}
% We aim to address Multi-Task Learning (MTL) with a large number of tasks by Multi-Task Grouping (MTG) techniques. Given $N$ tasks, we propose to \textbf{efficiently identify the best task groups from $2^N$ candidates and train the model weights simultaneously in one-shot}, with \textbf{the high-order task-affinity fully exploited}. This is distinct from the pioneering methods which either train numerous group candidates from scratch to discover the best one, or less precisely leverage pairwise tasks to approximate the high-order affinity. Moreover, our group identification and grouped task learning are unified and optimized using the final task losses directly in one shot, which differs from the separated procedures in common practice where the group identification often relies on heuristics. As a result, our method not only improves the training efficiency but also mitigates the objective bias that potentially leads to a suboptimal solution. We formulate MTG as a pruning problem on an adaptive network architecture that is fully differentiable. Specifically, given $N$ tasks for $K$ groups (\ie, $K$ encoder branches), we initially set up each branch to predict all the $N$ tasks to exploit the high-order task-affinity. Then, we gradually prune the $KN$ heads down to $N$ by gradients, ensuring that each task is exclusively and uniquely predicted by one branch. 
% Therefore, our model architecture is determined by a categorical distribution, which is then continuously relaxed to a concrete distribution and optimized by Gumbel softmax. Note that our pruning \emph{per se} is also efficient, as we only expand task heads rather than task-specific encoders. 
% Extensive experiments on XXX demonstrate XXX. The codes will be released.
We aim to address Multi-Task Learning (MTL) with a large number of tasks by Multi-Task Grouping (MTG) techniques. Given $N$ tasks, we propose to \emph{efficiently identify the best task groups from $2^N$ candidates and train the model weights simultaneously in one-shot}, with \emph{the high-order task-affinity fully exploited}. This is distinct from the pioneering methods which either train numerous group candidates from scratch to discover the best one, or less precisely leverage pairwise tasks to approximate the high-order affinity. Moreover, our group identification and grouped task learning are unified and optimized using the final task losses directly in one shot, which differs from the separated procedures in common practice where the group identification often relies on heuristics. As a result, our method not only improves the training efficiency but also mitigates the objective bias that potentially leads to a suboptimal solution. We formulate MTG as a pruning problem on an adaptive network architecture that is fully differentiable. Specifically, in order to categorize $N$ tasks into $K$ groups (\ie, $K$ encoder branches), we initially set up each branch to predict all the $N$ tasks to exploit the high-order task-affinity. Then, we gradually prune the $KN$ heads down to $N$ by gradients, ensuring that each task is exclusively and uniquely predicted by only one branch. Extensive experiments on CelebA and Taskonomy datasets with 5, 9, and 40 tasks demonstrate the promising performance and efficiency of our method. The codes will be released.
\end{abstract}



==> sec/1_intro.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth]{image/pruning.pdf}
    \vspace{-8mm}
    \caption{We formulate the Multi-Task Grouping (MTG) problem as network pruning. This figure illustrates the categorization of 4 tasks into 3 groups, where each branch represents a task group. As shown in the Upper Subfigure, at initialization, each group predicts all tasks, ensuring full exploration of high-order task-affinity. Throughout MTG training, we simultaneously prune the task heads and train the weights of the group-specific branches. Our training process ensures that MTG converges to a categorization where each task exclusively and uniquely belongs to only one group, as illustrated in the Lower Subfigure.}
    \label{img:pruning}
    \vspace{-3mm}
\end{figure}

\section{Introduction}
\label{sec:intro}

Many real-world applications are essentially complex systems that involve the collaboration of a large number of tasks. For example, in autonomous driving \cite{caesarnuscenes2020,huplanning2023}, in order to achieve good results with minimal human intervention, the autonomous driving system needs to simultaneously perform lane detection \cite{tangreview2021}, depth estimation \cite{godarddigging2019}, vehicle detection and instance segmentation \cite{maskrcnn,maskformer2021}, pedestrians localization \cite{bertonimonoloco2019}, etc. Therefore, to tackle these real-world challenges, it is crucial to simultaneously learn a large number of diverse tasks within a Multi-Task Learning (MTL) framework \cite{ubernet2017,lwr2019,blitznet2017,mtl2016,mtl3d2016,lirobust2021,wanggradient2021,liutowards2020,yugradient2020}, which reduces the inference time and facilitates an improved performance by leveraging the affinity among different tasks.



However, it is critical to carefully harness the affinity between those diverse tasks. Compared to learning them independently, simply combining them and feeding them into a fully-shared network oftentimes deteriorates the performance of several or even most tasks. Such phenomenon is attributed to the presence of the inherent \emph{negative transfer}, where the intuition is that the gradients from different tasks may interfere with each other when flowing into a shared encoder.

Pioneering works alleviate the negative transfer by designing novel Multi-Task Architectures (MTA) \cite{mtl1997,convexmtl2008,mtl2011,mtaoverview2017,mtaoverreview2021} or applying the Multi-Task Optimization (MTO) methods \cite{sener2018,lin2019,liuconflict2021,suteuregularizing2019,yangdeep2016}, where state-of-the-art MTA with soft-parameter sharing assigns independent network parameters to different tasks, while MTO directly manipulate the gradients from different tasks before applying them to update the shared parameters. However, both MTA and MTO methods pose challenges when scaling to a large number of tasks, \ie, the scalability is impeded in MTA for both training and evaluation due to the introduced extra parameters, while the training of MTO cannot maintain scalability either because it has to retain the gradients backward graphs for each task. Moreover, recent research suggests that it is difficult to address the negative transfer solely by manipulating gradients in MTO \cite{xin2022,kurin2022}.


We instead propose to facilitate a large number of tasks in MTL by Multi-Task Grouping (MTG). In MTG \cite{hoa2020,tag2021,mtg2022}, input tasks are categorized into groups by their affinity, where a group of tasks, as opposed to a single task, is modeled by a unique encoder. Consider categorizing $N$ tasks into $K$ groups, it significantly reduces the training complexity from $O(N)$ for MTA or MTO to $O(K)$ for MTG. Moreover, the grouping results of MTG naturally provide the interpretability of the task affinity, this is particularly desirable when the systems become extremely complex such as autonomous driving or recommendation systems.

The primary challenge of MTG is the exponential $2^N$ group candidates to be exhaustively trained from scratch, given merely $N$ tasks. In order to migrate this issue, Standley et al. \cite{hoa2020} and  Fifty et al. \cite{tag2021} propose to average the pairwise affinities to approximate the high-order affinities, \eg, the performance of Task $A$ in group $\{A, B, C\}$ can be obtained by averaging that of $A$ in $\{A, B\}$ and $\{A, C\}$. Despite a reduced complexity from $2^N$ to $N^2$, the less precise assumption of linear tasks affinity in \cite{hoa2020,tag2021} degrades the final performance. On the other hand, Song et al. \cite{mtg2022} advocate to train a meta-learner that directly predicts the final performance given a group candidate. However, the training of the meta-learner \emph{per se} is extremely difficult and involves collecting numerous well-trained group samples. Furthermore, existing methods perform group identification and grouped task learning in separated sequential procedures. As a result, the former potentially introduces objective bias \emph{w.r.t.} with the latter, especially when the groups are categorized based on heuristics. This also leads to a degradation in performance.

In view of those limitations, we propose to \emph{formulate MTG as a pruning problem of an adaptive network architecture}, as shown in Figure \ref{img:pruning}, which enables to i) \emph{identify the best groups and train the grouped model weights simultaneously in one-shot}, as well as ii) \emph{fully exploiting the high-order task affinities}. In our unified one-shot learning, we relate the group identification as the model architecture learning/pruning, and the grouped task learning is regarded as the model weights training under the current architecture. In this way, both procedures mutually facilitate each other to a better convergence. We jointly train both procedures by the final task losses, where the high-order task affinities are directly exploited. Our approach excels in both efficiency and accuracy, which is distinct from pioneering methods that first approximately identify grouping results, then train the grouped model from scratch subsequently.

Specifically, we formulate the categorization of $N$ tasks into $K$ groups as the learning of a \texttt{categorical} distribution, where the \texttt{categorical} distribution is related to our learnable network architecture. We then optimize the unified group identification and grouped task learning by leveraging a pruning algorithm that is fully differentiable. In order to do that, our method starts with $K$ branches, each equipped with $N$ heads, \ie, we evenly initialize the \texttt{categorical} distribution where each task has the same probability to be categorized into any group. It indicates that at the beginning, all the tasks are predictable by every group, ensuring full exploitation of the high-order task-affinity. After that, we optimize the model weights as well as the \texttt{categorical} distribution such that the $KN$ heads are gradually pruned down to $N$, facilitating that each task is exclusively and uniquely predicted by only one branch. Our \texttt{categorical} distribution is continuously relaxed then optimized by Gumbel softmax \cite{maddison2016concrete}. Note that our pruning procedure \emph{per se} is efficient, as we only expand \emph{the last task head layers} rather than \emph{task-specific encoders}. 

Our method has been extensively validated on CelebA \cite{faceattribute2015} and Taskonomy \cite{taskonomy2018} datasets with 5, 9, and 40 tasks, which demonstrates the promising performance and efficiency of our methods. Our method exhibits the following two unique features:
\begin{itemize}
\item \textbf{Efficiency}, which comes from i) our pruning formulation instead of sampling group candidates to train from scratch, and ii) the one-shot training that unifies group identification and grouped task learning.
\item \textbf{Accuracy}, which is ensured by i) fully exploiting the high-order task affinities within the \texttt{categorical} distribution, and ii) the elimination of the objective bias by the one-shot training of unified group identification and grouped task learning.
\end{itemize}


==> sec/2_related_work.tex <==
\section{Related work}
\label{sec: related work}

\subsection{Multi-Task Grouping}

It is expected to put collaborative tasks from a task pool into the same group to be learned by a hard-parameter shared network \cite{mtl2011,learningtg2012,jointgroups2021}.
Grouping tasks is able to efficiently learn a large scale of tasks, which is of high interpretation as well.
% It \cite{mtl2011,learningtg2012,jointgroups2021} can be split into two stages: group identification and grouped task learning. In the first stage, it is expected to put collaborative tasks in a task pool into the same group while separate competitive tasks. Afterward, grouped tasks are typically used to train a hard-parameter shared network.
% Grouping tasks before learning is able to alleviate negative transfer caused by competitive tasks so that networks can behave better on all learning tasks. Meanwhile, MTG is highly interpretable and efficient, especially on a large task-scale scenario. 
However, MTG is facing a dilemma in that it is prohibitive to search for an optimal grouping solution in $2^N-1$ task combination space. All of the current grouping methods \cite{hoa2020,tag2021,mtg2022} made attempts to model an evaluation function to figure out higher-order task relationships approximately from their low-order observations. 
% \% Standley et al. \cite{hoa2020} and Fifty et al. \cite{tag2021} linearly measured higher-order relationships from collected observations of pairwise task combinations, while Song et al. \cite{mtg2022} used a meta-learner to predict task relationships in arbitrary orders. They all consume too much time in modeling a measured function in terms of tasks.\% 
Furthermore, they separated group identification and grouped task learning and only considered low-order task affinity.
% Next, deriving the best grouping solution by certain search algorithms trains deep learning networks. 
Unlike them, our grouping approach integrates group identification and grouped task learning in one-shot training, greatly improving running efficiency on large task-scale scenarios as well as thoroughly considers higher-order task relationships. 
% It also effectively considers higher-order task relationships since different groups contain all learning tasks at initialization. 

\subsection{Multi-Task Architecture} 

Multi-Task Architecture \cite{mtl1997,convexmtl2008,mtl2011,mtaoverview2017,mtaoverreview2021} is a prevailing technology line in the Multi-Task Learnig domain. 
% It intends to design ingenious modules to avoid gradient conflicts in learning diverse tasks. 
It can be categorized as hard-parameter sharing \cite{ubernet2017,lwr2019,blitznet2017,mtl2016,mtl3d2016} and soft-parameter sharing \cite{nddr2019,crosslingual2015,crossstitch2016,mrn2017}. The former shares a common feature extraction module among tasks, while the latter assigns a special feature extraction branch for each task, exchanging features through extra fusion modules. 
% As a representative of hard-parameter sharing, UberNet \cite{ubernet2017} has succeeded in handling 7 computer vision tasks by sharing all parameters among them. For soft-parameter sharing, Cross-Stitch \cite{crossstitch2016} linearly fuses features from different task branches, and NDDR-CNN \cite{nddr2019} further designs a more general feature fusion mechanism, namely neural discriminative dimensionality reduction. 
% Representative models, such as UberNet \cite{ubernet2017} and NDDR-CNN \cite{nddr2019}, have succeed in handling multiple vision tasks cooperatively.
They are unable to work in a large task-scale case, although their success proved it is feasible to address MTL through appropriate network structure modification. This is because hard-parameter sharing \cite{vandenhende2019,learntobranch2020,bruggemann2020,adashare2020} is hard to avoid negative transfer owing to a full-shared feature module especially when more tasks are learned. In soft-parameter sharing \cite{ruderlatent2019,zhangjoint2018,padnet2018,zhangpattern2019}, parameter numbers linearly grow with tasks, which better deal with the negative transfer but introduce heavier inference costs.

\subsection{Multi-Task Optimization} 
Multi-Task Optimization develops in parallel with Multi-Task Architecture, which aims to adjust task loss by balancing task uncertainty \cite{uncertainty2018}, normalizing gradients \cite{gradnorm12018,gradnorm22019}, weighting tasks randomly \cite{weightingtask12022,weightingtask22020}, and rearranging task priority \cite{rearranging2018} so that the learning progresses of different tasks are uniform. In recent years, more and more studies \cite{lirobust2021,wanggradient2021,liutowards2020,yugradient2020} have begun to straightforwardly correct gradients to mitigate conflicts in training, e.g., projecting task gradients when their angle is greater than $90^{\circ}$. Revising gradients, in practice, requires taking more memory to store the gradient graph for each task, which is infeasible when working with a large number of tasks. And now, on the basis of extensive experiment observations, Kurin et al. \yrcite{kurin2022} and Xin et al. \yrcite{xin2022} pointed out that current MTO is not always superior to methods that simply weight all task loss. Thus, it is necessary to find another more efficient and effective modeling method to optimize MTL.

\subsection{Network Pruning} 

Network pruning \cite{caiproxylessnas2018,chenreinforced2018,elskenneural2019,ghiasifpn2019,hemilenas2020,lipartial2019} aims to cut out unnecessary neural connections with little model degradation. This pruning process can be implemented by Bayesian optimization \cite{makingbergstra2013}, evolutionary algorithms \cite{regularizedreal2019,xiegenetic2017}, network transformation \cite{elskensimple2017,gordonmorphnet2018}, reinforcement learning \cite{irlasguo2019,mnasnettan2019,learningzoph2018}, and gradient descent \cite{akimotoadaptive2019,liuauto2019,wufbnet2019,zhangcustomizable2019}. 
% From the view of pruning objects, network pruning can be divided into weight pruning, neuron pruning, layer pruning, and structural pruning. Our approach regards task grouping as a structural pruning process, where different groups start with all task heads and gradually drop out competitive heads until converging. 
We use differentiated pruning operations, which effectively enable integrating group identification with grouped task learning in joint training. Consequently, group identification and grouped task learning that are optimized by the same loss avoid their objective bias in training. 
% Before us, network pruning is only considered as a lightweight tool for deep learning models. 
We are the first to combine it with MTG to unify group identification and grouped task learning in an end-to-end architecture.

% \textbf{Multi-task Grouping.} The motivation for multi-task grouping \cite{hoa2020, tag2021, mtg2022} is to group related tasks to train jointly so that they can benefit from the inductive bias of each other and behave better after multi-task learning. It would also eliminate negative transfer incurred by competitiveness between unrelated tasks from multi-task learning. So multi-task grouping is a significant premise step before conducting multi-task learning. But how to evaluate which tasks are cooperative and which tasks are competitive is hard since their correlation is highly non-linear and we are unable to interpret them in detail when more tasks are introduced. One straightforward method is traversing all task combinations to train a deep learning model individually and finds the best groupings among them, which has an exponential search space related to the number of tasks. The prohibitively expensive computation cost of training models on such a large space restricts it to group a small range of tasks. Thus, designing an effective and efficient grouping method that is competent to work on a large range of tasks for deep learning models is an obstacle to multi-task grouping.

% The early attempt \cite{hoa2020} in this field first formally divided multi-task grouping for deep learning models into two stages: 1) efficiently measuring correlations across tasks based on a function related to tasks, and then 2) searching for optimal task grouping in accordance with previously computed correlations. In the first stage, Standley et al. \cite{hoa2020} defined task correlation as their transfer gain (or gain prediction) and obtained second-order transfer gains on training models over all pairwise task combinations. Afterward, they approximately calculated higher order transfer gains over three and more tasks through a linearly weighted average of second-order solutions of their pairwise combinations, which is so-called higher order approximation (HOA). Next, an optimal grouping can be found when obtaining transfer gains about tasks in all orders, and those tasks in the same group are used to re-train models together. Although approximating higher order solutions via a low order linear combination can greatly save much training time, task correlation as mentioned above is highly non-linear, and only pairwise relationships are considered here. 

% Following the defined workflow, Fifty et al. \cite{tag2021} proposed task affinity grouping (TAG) that replaced transfer gains with gradients to quantify task correlation and trained all tasks in a run to identify task groupings with a maximum total inter-task affinity. Song et al. \cite{mtg2022} randomly sampled some task combinations and their transfer gains, which were used to learn a measured function via meta-learning so as to generalize it to other combinations. Despite the success of existing approaches in multi-task grouping, they always separated grouping and learning into two individual phases, and their metrics (transfer gains and gradients) for grouping are model-driven. Once model architecture changes, these metrics may change together since some models may include special modules friendly for certain tasks but not for others. Experiments in \cite{tag2021} also demonstrate that hyperparameter setups would also influence task grouping. As a result, the grouping results determined on the model can not be transferred to another. However, our approach integrates multi-task grouping with learning in an end-to-end manner, alleviating their gap. After finishing training, task groupings and their corresponding models have been learned at the same time. Besides, all tasks are incorporated into the training so that it can consider complex task relationships to make a more convinced decision.  

% \textbf{Multi-task Learning.} Previous to the emergence of multi-task grouping, multi-task learning \cite{mtl1997,convexmtl2008,mtl2011} has been studied for a long time from different perspectives, such as hard parameter sharing \cite{ubernet2017,lwr2019,blitznet2017,mtl2016,mtl3d2016}, soft parameter sharing \cite{nddr2019,crosslingual2015,crossstitch2016,mrn2017}, and neural architecture search (NAS) \cite{mtlnas2020,learntobranch2020,adashare2020,mtlevolutionary2018}, which is prevailing and important in computer vision especially when deep learning that has abundant parameters becomes popular. It attempts to learn multiple tasks jointly by a deep learning model so as to improve running efficiency to be adapted in situations with limited resources and computation as well as quick response to several tasks, such as autonomous driving. It is also desired that the model trained with multiple tasks perform better than training on a single task owing to information sharing across these tasks. As the most famous representative of the hard parameter sharing technology recently, UberNet \cite{ubernet2017} directly shares all parameters of the model among tasks and has successfully handled 7 computer vision issues. Nevertheless, it would suffer from performance degradation caused by negative transfer, as more and more tasks are added into training without considering their competitiveness. This makes training deep learning models to simultaneously learn diverse tasks and benefit from each inductive bias more challenging.

% To alleviate the dilemma, other methods, such as soft parameter sharing and neural architecture search, adaptively determine which parts of the model's parameters should be shared across tasks and which parts should not. Soft parameter sharing approaches typically train a task-specific branch for each task as well as a sharing mechanism among them so that they can selectively fuse useful information from others instead of using the same set of parameters to extract common features for distinct tasks. Learning task features from separated branches in parallel and interacting with others via a soft sharing mechanism is straightforward to mitigate negative interference coming from competitive tasks, but the total number of parameters would increase linearly with the task number. This linear increase can not be negligible since current models usually have millions of parameters. Additionally, increasing the task number would also make the feature interaction between tasks become more complex. Another method intends to find appropriate paths in a single model for different tasks via NAS \cite{nas2018,darts2018,snas2018}, dropping out competitive components finally. 

% From the view of multi-task learning, the proposed method totally includes $K$ times multi-tasks, where $K$ is the group number, and tries to find optimal paths during training like NAS. We differ in searching within the loss layer, rather than the model layers, to group related tasks within the same branch for joint learning while preventing gradient backward propagation for unrelated tasks in that branch.



==> sec/3_method.tex <==
\section{Method}
\label{sec:Method}

\begin{figure*}[t]
% \vspace{5mm}
    \centering
    \includegraphics[width=\textwidth]{image/framework.pdf}
    \vspace{-7mm}
    % \caption{The overview of our method. We formulate the Multi-Task Grouping (MTG) problem as network pruning, where our method consists of a grouped task learning module and a group identification module. In order to categorize $N$ tasks into $K$ groups, our network is constructed with $K$ group-specific branches, optionally with shared lower layers. We illustrate in this figure for categorizing 3 tasks into 2 groups.}
    \caption{The overview of our method. We formulate the Multi-Task Grouping (MTG) problem as network pruning, where our method consists of a grouped task learning module and a group identification module. In order to categorize $N$ tasks into $K$ groups, our network is constructed with $K$ group-specific branches, optionally with shared lower layers. At initialization, we enable each branch to predict all tasks, so that the high-order task-affinity can be exploited. We then relate the grouped task learning to the model weights training of each group-specific branch, and the group identification as the model head/loss pruning. The final grouped task losses are generated by both modules, which in turn ensures that both modules can be trained simultaneously. As a result, our method is able to learn the group identification and the grouped model weights in one-shot, with the high-order task-affinity fully exploited. We illustrate in this figure for categorizing 3 tasks into 2 groups.}
    \label{img:framework}
    % \vspace{5mm}
    \vspace{-3mm}
\end{figure*}

In the paper, we address Multi-Task Learning (MTL) with a large number of tasks by Multi-Task Grouping (MTG), where a shared encoder is assigned to each group of tasks. Consider categorizing $N$ tasks into $K$ groups, MTG effectively reduces the training complexity of widely used MTL techniques, such as Multi-Task Architecture (MTA) \cite{nddr2019,crosslingual2015,crossstitch2016,mrn2017} and Multi-Task Optimization (MTO) \cite{lirobust2021,wanggradient2021,liutowards2020,yugradient2020}, from $O(N)$ to $O(K)$.

MTG consists of two primary procedures, where \emph{group identification} categorizes the collaborative tasks into the same group, while \emph{grouped task learning} is to train the model weights given the grouping results \cite{hoa2020,tag2021}. Given $N$ tasks, the main challenge of MTG is the exponentially large $2^N$ grouping candidates for group identification \cite{hoa2020,tag2021,mtg2022}.

We propose to efficiently chase the best grouping results from the $2^N$ candidates with \emph{the high-order tasks affinities directly exploited}. To this end, we \emph{formulate MTG into a network pruning framework}, where we relate \emph{the group identification as the model architecture learning/pruning, and the grouped task learning as the model weights optimization under certain architecture}. As a result, the group identification and the grouped task learning are unified and can be jointly optimized in one-shot during network pruning. 

Regarding the optimization process, we treat the group categorization as a \texttt{categorical} distribution, which is then continuously relaxed into a \texttt{concrete} distribution and subsequently optimized using the Gumbel softmax \cite{maddison2016concrete}. It is worth noting that our pruning method is also efficient because we only expand task heads rather than task-specific encoders.

The merits of our formulation are three-fold: i) It enables us to exploit the high-order task affinities directly. ii) It avoids the potential objective bias when group identification and grouped task learning act as separated sequential procedures. In other words, the group identification results obtained through heuristics when training \emph{all the $N$ tasks}, such as task-wise conflict-gradients \cite{tag2021}, may not be appropriately used to train \emph{a group subset of tasks} from scratch. This is because the grouped tasks may conflict again without the influence of other tasks. iii) The pruning algorithm directly produces a well-trained and grouped network that is readily for inference, without the need of retraining from scratch.

\subsection{Problem Formulation}
Formally, we consider categorizing a set of $N$ tasks $\mathcal{T} = \{\mathcal{T}_{1}, ..., \mathcal{T}_{N}\}$ into equal or less than $K$ groups $\mathcal{G} = \{\mathcal{G}_{1}, ..., \mathcal{G}_{K}\}$, such that each group contains 0 to $N$ tasks $\mathcal{G}_k = \{..., \mathcal{T}_{i}, ... \}$, and each task is exclusively and uniquely belongs to one group. Therefore, we have:
\begin{align}
    &\mathcal{T} = \cup _{k=1}^{K} \mathcal{G}_{k}, \notag \\
    s.t. \quad &\forall k, \quad |\mathcal{G}_k| \in \{0, ..., N\}, \nonumber \\ 
    &\forall (i, j), \quad \mathcal{G}_{i}\cap \mathcal{G}_{j}=\emptyset,
    \label{eq:grouping}   
\end{align}
where $|\cdot|$ is the cardinality. We optimize our problem exclusively to attain the highest average performance across these $N$ tasks, without relying on auxiliary heuristic criteria. We also note that $K$ is the maximal-allowed number of groups as determined by the training budget, and we do not impose a strict requirement to yield precisely $K$ groups, \ie, some groups may contain 0 task.

% Moreover, our grouping process is entirely governed by the loss function during training, \emph{i.e.,} fitting an evaluation function to predict grouping performance like current all works is unnecessary here, the fitness of which would highly influence subsequent multi-task learning. There is no need to search for the best grouping solution since our grouping result is determined once the training is complete. 

% Next, we first give an overview of our proposed method. Then, we will detail how MTG is conducted by adaptively pruning competitive task heads to minimize training loss. Finally, constructing a network adapts to our grouping process so that MTG and MTL are seamlessly coupled to train in one-shot, which significantly increases the scalability and robustness of our architecture in cases with a large number of tasks.

% As our grouping mechanism is differentiated and influenced by gradients, it can reflect a comprehensive grouping result led by task relationships, network choices, parameter initialization, and so on.



% \subsection{Overview}
As shown in Figure \ref{img:framework}, our method comprises a grouped task learning module and a group identification module. These two modules complement each other and can be trained jointly. Specifically, during the training for each group of tasks, the group identification module selects collaborative tasks to back-propagate gradients to the correct branch of the grouped task learning module. Each branch of the grouped task learning module is responsible for one group, which in turn facilitates group identification.

We detail the grouped task learning module, the group identification module, and the joint optimization in the following sections.


\subsection{Grouped Task Learning Module} 

We formulate $K$ branches in the grouped task learning module, where each branch represents the encoder of each task group. We relate the model weights training of each group branch to the grouped task learning.

Our method also optionally contains group-shared layers before splitting into the group-specific branches, which can be used to further compress the network size.


\subsection{Group Identification Module Formation}

We consider categorizing $N$ tasks exclusively and uniquely into $K$ groups as the learning of a \texttt{categorical} distribution, and we relate the learning of the \texttt{categorical} distribution to adaptive network architectures. As such, the underlying \texttt{categorical} distribution can be optimized jointly with the model weights, which we formulate as a pruning problem.

\noindent \textbf{\texttt{Categorical} Distribution.} Formally, let a random variable $z_{ik}$ indicate the assignment of task $i$ to group $k$, which is sampled from some discrete distribution. In order to assign $N$ tasks to $K$ groups, we have a set of random variables $Z = \{z_{ik} \} \in \mathbb{R}^{N \times K}$. 

Recall Eq. \eqref{eq:grouping} that each task is exclusively and uniquely categorized into one group, therefore, we have:
\begin{equation}
    \sum_k z_{ik} = 1, \qquad \text{and} \qquad z_{ik} \in \{0, 1\}, \quad \forall k,
    \label{eq:k_row}   
\end{equation}
which indicate that each row of $Z$ follows a \texttt{categorical} distribution. Let the \texttt{categorical} random variable $z_{ik}$ be parameterized by $s_{ik}$, \ie:
\begin{equation}
    z_{ik} \sim \texttt{Categorical}(s_{ik}),
    \label{eq:cate}   
\end{equation}
where $s_{ik}$ represents the probability of assigning task $i$ to group $k$.

\noindent \textbf{Network Architecture.} We relate the \texttt{Categorical} Distribution to the network architecture and formulate a pruning problem so that the Group Identification Module and the Grouped Task Learning Module can be optimized jointly.

To achieve that with minimal additional complexity, we formulate the sampled random variable $z_{ik}$ as the loss indicator, which determines whether to back-propagate the loss of task $i$ to the $k$-th group. Specifically, we connect each of $K$ group encoders to each of $N$ task heads, resulting in loss matrix $L = \{L_{ik} \} \in \mathbb{R}^{N \times K}$. The final loss for back-propagation can be obtained by:
\begin{equation}
    L^{\text{task}}(\theta, S) = L(\theta) \odot Z(S),
    \label{eq:loss}
\end{equation}
where $\odot$ is the element-wise product, $\theta$ is the model weights, and $S = \{ s_{ik} \} \in \mathbb{R}^{N \times K}$ is the set of parameters of the \texttt{categorical} distributions.

As shown in Eq. \ref{eq:loss}, we formulate MTG as a pruning problem where $Z(S)$ is learned to prune the $KN$ losses $L(\theta)$. Since we only expend the task heads rather than the encoder, our pruning \emph{per se} is also efficient.


\subsection{The Joint Optimization}
Equation \eqref{eq:cate} indicates a discrete sampling from $s_{ik}$ to $z_{ik}$, which results in a gradient blockage in Eq. \eqref{eq:loss} when back-propagate the gradient from $Z$ to $S$. In this section, we relax the discrete \texttt{categorical} distribution to be continuous, so that both the parameters for group identification $S$ and the parameters for grouped task learning $\theta$ can be optimized by gradients from the task loss $L^{\text{task}}(\theta, S)$ through $Z(S)$ and $L(\theta)$, respectively.

\noindent \textbf{Continuous Relaxation.} By using the reparameter trick from the \texttt{Concrete} distribution \cite{maddison2016concrete}, we are able to continuously sample $s_{ik}$ to produce $\tilde{z}_{ik}$ that approximate $z_{ik}$ in \texttt{Categorical} distribution. This enables the gradient flow from $\tilde{z}_{ik}$ to $s_{ik}$. The reparameterized \texttt{Categorical} distribution can be modeled by the differentiable Gumbel softmax, \ie:
\begin{equation}
    \tilde{z}_{ik} = \frac{\exp((s_{ik}+g_{ik})/\tau)}{\sum _{m=1}^{K}\exp((s_{im}+g_{im})/\tau)}
    \label{eq:gumbel}
\end{equation}
where $g_{ik}$ is sampled from a \texttt{Gumbel} distribution, \ie, $g_{ik}=-\log(-\log(\texttt{Uniform}(0, 1)))$ \cite{maddison2016concrete}. $\tau$ is a temperature that controls the shape of the output distribution. $\tau$ is annealed to $0$ during the training, resulting in a discrete $\tilde{z}_{ik}$ as a good approximation of $z_{ik}$. Then, the loss in Eq. \eqref{eq:loss} becomes:
\begin{equation}
    L^{\text{relaxed task}}(\theta, S) = L(\theta) \odot \widetilde{Z}(S),
    \label{eq:relaxed_loss}
\end{equation}
where $\widetilde{Z} = \{ \tilde{z}_{ik} \} \in \mathbb{R}^{N \times K}$.

% \noindent \textbf{Minimal Entropy Regularization.} Despite that $\tilde{z}_{ik}$ is precisely binary when $\tau$ is annealed to 0, directly optimize Eq. \eqref{eq:relaxed_loss} does not necessarily produce a binary $s_{ik}$. Consequently, this leads to a large variance when sampling $\tilde{z}_{ik}$ by Eq. \eqref{eq:gumbel}. As an extreme case, a converged $s_{ik} = 1/K, \forall k$ produces a random guess to categorize task $i$ to any group, as shown in XXX.

% Therefore, minimal entropy regularization on $s_{ik}$ is employed to push $s_{ik}$ to be binary, which effectively reduces the sampling variance of $\tilde{z}_{ik}$. As a result, this not only stabilizes the training procedure but also produces a meaningful grouping result. We use symmetric minimal entropy regularization as:
% \begin{equation}
%     L^\text{entropy} = \frac{1}{N}\sum_{i=1}^{N}\sum_{k=1}^{K}\{-s_{ik}\log s_{ik}- (1-s_{ik})\log(1-s_{ik})\}
%     \label{eq:entropy}
% \end{equation}

% \noindent \textbf{Final Objective and Initialization.} Our final objective is:
% \begin{equation}
%     L^\text{final} = L^\text{relaxed task} + \lambda L^\text{entropy},
%     \label{eq:final}
% \end{equation}
% where $L^\text{relaxed task}$ and $L^\text{entropy}$ come from Eqs. \eqref{eq:relaxed_loss} and \eqref{eq:entropy}, respectively. $\lambda$ is a weight parameter to balance the two losses.

\noindent \textbf{Initialization.} We note that the parameter of the \texttt{categorical} distribution, $s_{ik}$, can be initialized according to the prior knowledge of the task affinity. In our problem, we simply initialize each $s_{ik}$ to $1/K$, which implies that each task may be evenly categorized into any group. In other words, we do not assume any task affinities and fully learn them from data. Therefore, the optimization of our model can be viewed as pruning initially $KN$ task heads to $N$, where each task is exclusively and uniquely categorized to one group after convergence.

\subsection{Evaluation Metrics}  \label{sec:metrics}
Pioneer research commonly relied on the \emph{total loss} as the evaluation metric \cite{hoa2020,tag2021,mtg2022}, which straightforwardly sums up the losses of all tasks. However, the magnitudes of losses from different tasks significantly vary due to i) different loss types, such as cross-entropy losses for classification and $\ell_{1}$ losses for regression, and ii) diverse labels, such as image-level classification labels and pixel-level semantic segmentation labels. Consequently, simply calculating the \emph{total loss} may lead to an overestimation of tasks with higher loss magnitudes while obscuring those with lower loss magnitudes. 

For example, in the Taskonomy experiments, the semantic segmentation loss exhibits two orders of magnitude higher than the depth estimation loss. When using \emph{total loss} as a metric, even a slight improvement in semantic segmentation can overshadow a significant degradation in depth estimation. This phenomenon contradicts the the fundamental goal of MTG, which is to boost \emph{all the input tasks rather than a subset of them} \cite{hoa2020}.

To comprehensively assess improvements of a MTG method across all tasks, we eliminate the influence of loss magnitudes by employing a new evaluation metric termed \textbf{normalized gain}. Specifically, we initially calculate the normalized loss improvement (expressed as a percentage) \emph{w.r.t.} the naive MTL architecture (\ie, the shared-encoder architecture) for each task, then average them across all tasks:
\begin{equation}
    \text{NormGain}_{L} = \frac{1}{N}\sum_{n=1}^{N}\frac{L^{\text{task } n}_\text{MTL}-L^{\text{task } n}_\text{method}}{L^{\text{task } n}_\text{MTL}},
    \label{eq:taskonomy error}
\end{equation}
where $L$ denotes loss and $N$ is the total number of tasks. Similarly, in cases where a unified evaluation is applicable for all input tasks (\eg, classification error when all input tasks are classifications), we can also present \textbf{normalized gain} \emph{w.r.t.} such unified evaluation error:
\begin{align}
    &\text{NormGain}_{E} = \frac{1}{N} \sum_{n=1}^{N} \frac{E^{\text{task } n}_\text{MTL} - E^{\text{task } n}_\text{method}}{E^{\text{task } n}_\text{MTL}}, 
    \label{eq:classification error}
\end{align}
where $E$ denotes the unified evaluation error.

 % a shared backbone across all tasks, group-bones shared by those tasks in the same group, task heads to decode corresponding outputs, a loss layer to calculate task loss from different groups respectively, and a grouping layer to divide $N$ tasks into no more than $K$ groups. The first three modules take responsibility for multi-task learning, and the last conducts multi-task grouping by fitting a categorical distribution to prune conflict heads. 

% During training, the grouping layer, adjusted by backward gradients, learns which tasks should be grouped together for multi-task learning and which tasks should not.

% Specifically, given an input image $I$, it would be transmitted into a shared backbone to extract common features across all tasks. These common features are copied $K$ times and input into every $\text{group-bone}_{k}, k=1,\dots,K$. Subsequently, $N$ task heads behind each $\text{group-bone}_{k}$ would take its output as input and generate corresponding task predictions. These task predictions across groups are aggregated by the loss layer to calculate their loss compared to ground truths, resulting in a loss matrix $\mathbf{L}\in \mathcal{R}^{N\times K}$. The row dimensions of the matrix correspond to tasks, while the column dimensions correspond to groups. So, the element at an index of $(n, k)$ is the loss value over the $n$-th task and $k$-th group. Finally, the grouping layer, parameterized by a learnable matrix $\mathbf{G} \in \mathcal{R}^{N\times K}$, samples a discrete grouping result $\widetilde{\mathbf{G}}$ through the gumbel-softmax operation. This then is element-wise weighted by the loss matrix to obtain the final loss.

% For the convenience of readers to understand our modeling approach more clearly, we have adjusted the order of introductions to multi-task learning and multi-task grouping. Next, we will first describe the grouping mechanism and then explain how the model is constructed to adapt to the former and perform grouped multi-task learning.

% \subsection{Learn to group tasks}
% Previous grouping methods aim to find an optimal grouping solution covering all $N$ tasks under the inference time cost restriction, but tolerate different groups containing the same tasks. During inference, each task is assigned to the model that achieves the highest test performance for it. Thus, even if the best grouping solution is found, it may not specify which model should perform which task. This dilemma arises from their relaxed solution that allows for the same task to be in different groups.

% To address the issue, we impose a stronger restriction on the final grouping result, requiring that each task must only belong to one of the $K$ groups. Formally, we want to divide $N$ tasks into $K$ groups, and these groups do not overlap each other, as shown in Equation \eqref{eq:grouping}:

% Every group $\mathcal{G}_{k}=\{\mathcal{T}_{n}\}$ includes certain tasks in $\mathcal{T}$. The relationships among $N$ tasks and $K$ groups in the grouping layer are represented by a parameterized grouping matrix $\mathbf{G}\in \mathbb{R}^{N\times K}$, which is trainable as well. Each element $\theta _{n, k}$ in the matrix indicates a probability that the $n$-th task belongs to the $k$-th group. Meanwhile, the elements at each row should sum to $1$, denoted as:
% \begin{equation}
%     \sum _{k=1}^{K} \theta _{n, k} = 1
%     \label{eq:sumtoone}
% \end{equation}
% In order to specify which task should be learned and performed by the model in the $k$-th group, they must follow a one-hot distribution, where only one element is equal to $1$ while others are $0$. The constraint in Equation \eqref{eq:sumtoone} can be achieved by row-wisely applying ${\rm softmax}(\cdot)$ to the grouping matrix. Furthermore, minimizing row-wise entropy can discretize each row into a one-hot distribution in the end.

% Nonetheless, one question is coming: how to initialize the grouping matrix? At the beginning, we don't know which tasks to group or which tasks can be grouped together. Therefore, the best initialization solution is assigning an even probability of $1/K$ to each group. Thus, at the initialization stage,
% \begin{equation}
%     \theta _{n, k} = \frac{1}{K}
% \end{equation}
% To enable a categorical distribution for $N$ tasks over $K$ groups, we use Gumbel Softmax to sample grouped outcomes from the parameterized grouping one at training, which is
% \begin{equation}
%     \widetilde{\theta}_{n, k} = \frac{exp((\theta _{n, k}+g_{n, k})/\tau)}{\sum _{i=1}^{K}exp((\theta _{n, i}+g_{n, i})/\tau)}
% \end{equation}
% Here, $g_{n, k}$ is sampled from the Gumbel distribution, where $g_{n, k}=-log(-log(u_{n, k}))$ and $u_{n, k}\sim U(0,1)$. $\tau$ is a temperature variable that controls the shape of the output distribution. When it annealed to $0$, the output distribution becomes a one-hot distribution to some extent. So, we can gradually decrease $\tau$ to make the output more discrete when training. The Gumbel Softmax also satisfies our analysis above, and, more importantly, it is differentiated so that coupling MTG and MTL in an architecture becomes possible.

% After sampling a discrete grouping matrix, it is weighted by the loss matrix to calculate the final loss, denoted as
% \begin{equation}
%     loss = {\rm sum}(\mathbf{L}*\widetilde{\mathbf{G}})
% \end{equation}
% % Owing to the discrete grouping matrix, each group only receives certain task gradients to update their parameters so as to conduct grouped multi-task learning. 
% In backward propagation, the parameterized grouping matrix would receive gradients with respect to each element $\theta _{n, k}$ to update. Assuming $loss_{n}$ is a total loss about the $n$-th task over $K$ groups, it can be calculated as:
% \begin{equation}
%     loss_{n} = \sum _{k=1}^{K} \widetilde{\theta}_{n, k}l_{n, k}
% \end{equation}
% Consequently, the gradient of $loss_n$ with respect to $\theta _{n, k}$ is
% \begin{align}
%     \frac{\partial loss_{n}}{\partial \theta _{n, k}} &= \frac{1}{\tau}[l_{n,k}\widetilde{\theta}_{n,k}(1-\widetilde{\theta}_{n,k})-\sum _{i=1, i!=k}^{K}l_{n,k}\widetilde{\theta}_{n,i}\widetilde{\theta}_{n,k}] \notag \\
%     &=\frac{\widetilde{\theta}_{n,k}}{\tau}(l_{n,k}-\sum _{i=1}^{K}l_{n,i}\widetilde{\theta}_{n,i})
%     \label{eq:gradient}
% \end{align}
% Since $\widetilde{\theta}_{n,k}\ge 0$ and $\tau >0$, the first term in the Equation \eqref{eq:gradient} must be greater than $0$. So, whether the gradient is positive or negative depends on its second term. If $l_{n,k}$ is the current minimum among $\{l_{n,i}\}_{i=1}^{K}$, it must be negative because of
% \begin{equation}
%     \sum _{i=1}^{K}l_{n,i}\widetilde{\theta}_{n,i}\ge l_{n,k}\sum _{i=1}^{K}\widetilde{\theta}_{n,i}=l_{n,k}
% \end{equation}
% As a result, updating $\theta _{n,k}$ with its negative gradient must lead to a greater grouping weight, indicating that this task should be divided into the $k$-th group. This also corresponds to its minimum loss behavior on the $k$-th group, where collaborative tasks are correctly assigned to learn. Otherwise, positive gradients would decrease the grouping weights. This is aligned with the higher loss in the group, indicating that current tasks learned in the group are competitive. As training progresses, each row in our grouping matrix would be a categorical distribution, representing that initial $KN$ task heads are gradually cut into final $N$ heads. Empirically, our method would converge to a group number less or equal to $K$, while other existing methods always group tasks into $K$ compulsively. So a exact $K$ is unnecessary for our method.

% As the above analysis, the evolution direction of the grouping matrix under the guidance of gradients conforms to our expectations very much. That is, it would seek an optimal group in which collaborative tasks remain in the same group and competitive ones are cut out so as to minimize the final loss. In training, Gumbel Softmax always needs a well-designed $\tau$ and more epoches to achieve convergence. To mitigate this issue, a minimal entropy penalty is applied on the parameterized grouping matrix that
% \begin{equation}
%     L_{entropy} = \frac{1}{N}\sum_{n=1}^{N}\sum_{k=1}^{K}-\theta_{n,k}log\theta_{n,k}-(1-\theta_{n,k})log(1-\theta_{n,k})
% \end{equation}
% Thus, our final loss is
% \begin{equation}
%     L=loss + \lambda L_{entropy}
% \end{equation}
% where $\lambda$ is a balance factor.

% \subsection{Learn to learn grouped task}
% To integrate multi-task grouping with multi-task learning in joint training, the model structure must adapt to the grouping matrix so that grouped outcomes can directly guide multi-task learning. To this end, we would instantiate $K$ networks, and each of them is independently followed by a set of $N$ task heads to decode task outputs. These outputs then are transmitted into the loss layer to calculate the loss matrix, which is weighted by a discrete grouping matrix to get the final loss. Task gradients in backward propagation would be filtered by the discrete grouping matrix and flow into assigned groups. As a result, every group learns only certain tasks assigned to it by the grouping matrix actually.

% Although competitiveness typically exists among tasks, they all have a common shallow feature set, such as colors, directions, lines, and so on. Therefore, we split the networks into two parts, which are named as \textbf{shared backbone} and \textbf{group-bone} respectively. The former is responsible for learning features shared across groups, while the latter intends to learn features shared by tasks within the same group. In practice, we use benchmark networks from \cite{hoa2020, tag2021} as our feature encoder. 
% % These two networks are built on a variant of Xception \cite{xception2017} and Resnet18 \cite{resnet2016} respectively. 
% These benchmarks are split into two parts by a customized split point $m$. As a result, their first $m$ layers become the shared backbone in Figure \ref{img:framework}, while correspondingly the remaining layers are the group-bone. The group-bone then copies $K$ times to correspond to the group dimensionality of the grouping matrix.
% % We set a split point $m$ where the first $m$ layers of the network serve as the shared backbone, while the remaining layers constitute the group-bone. Specifically speaking, one shared backbone and $K$ group-bones are instantiated for feature extraction between and within groups. 
% Additionally, each group-bone is associated with a set of heads covering all tasks. All in all, with the above designs, our architecture can learn multi-task grouping and multi-task learning concurrently. After training, task groups and their corresponding trained network are shown.

==> sec/4_experiments.tex <==
\section{Experiments}
\label{sec:Experiments}
In this section, we extensively validate our method on both \textbf{Taskonomy} \cite{taskonomy2018} and \textbf{CelebA} \cite{faceattribute2015} datasets for various candidate groups. We detail the experimental setup in the following.

\subsection{Experimental Setup}

\noindent \textbf{Datasets.} We perform experiments on Taskonomy \cite{taskonomy2018} dataset following \cite{hoa2020,tag2021,mtg2022}, and CelebA \cite{faceattribute2015} dataset following \cite{tag2021}. We use the official tiny train, validation, and test split of Taskonomy. The images from Taskonomy and CelebA are bilinearly downsampled to $256\times 256$ and $64\times64$, respectively as those in \cite{hoa2020,tag2021,mtg2022} and \cite{tag2021}.

\noindent \textbf{Benchmark Experiments.} We follow the experiment setups in \cite{hoa2020,tag2021,mtg2022} to conduct $5$ tasks on Taskonomy, \ie, \textit{semantic segmentation}, \textit{depth estimation}, \textit{surface normal}, \textit{keypoint detection}, and \textit{edge detection}, denoted as Taskonomy-$5$. We also conduct $9$ tasks on CelebA dataset following \cite{tag2021}, \ie, \textit{5\_o\_Clock\_Shadow}, \textit{Black\_Hair}, \textit{Blond\_Hair}, \textit{Brown\_Hair}, \textit{Goatee}, \textit{Mustache}, \textit{No\_Beard}, \textit{Rosy\_Cheeks}, and \textit{Wearing\_Hat}, referred to as CelebA-$9$.

\noindent \textbf{Network Backbone.} We use the same network backbone as \cite{hoa2020,tag2021}, \ie, a variant of Xception network \cite{xception2017}, for the Taskonomy experiments. While for the CelebA experiments, we use a variant of ResNet \cite{resnet2016} following \cite{tag2021}.

\noindent \textbf{Optimization.} We use Adam optimizer for all of our experiments, where the initial learning rates are $0.0008$ and $0.0001$ for the CelebA and Taskonomy experiments, respectively. We use \emph{plateau} learning rate decay which reduces by $0.5$ when the validation loss no longer improves. We train all the experiments for $100$ epochs, where our networks are initialized by the pretrained naive MTL weights on the corresponding experiments. We copy the networks and the group-specific parameters for $K$ times to ensure that the same task is initialized identically across different groups. We set the Gumbel Softmax parameter $\tau$ of Eq. \eqref{eq:gumbel} as $2.5$ and $4$ for the CelebA and Taskonomy experiments, respectively. We follow \cite{tag2021} to use the cross-entropy loss for the CelebA experiments, and follow \cite{hoa2020,tag2021} to use the cross-entropy loss for semantic segmentation and $\ell_{1}$ loss for other tasks of the Taskonomy experiments. 

% On the more challenging taskonomy dataset, we first follow the original configuration specified in \cite{taskonomy2018} to train a naive MTL model on all tasks from scratch, which is used to initialize our grouping model later. The initialized model, in conjunction with a learnable grouping matrix, undergoes joint training under 

% For the Taskonomy-5 experiment, we use the Adam optimizer with a learning rate of  for dozens of epochs, where $\tau$ is fixed as $4$. Meanwhile, a learning rate scheduler is adopted here to reduce the learning rate . The semantic segment task is supervised by corss-entropy loss, while others are supervised using the $\ell_{1}$ loss. The best parameters for each branch are saved based on their evaluation in the validation dataset.

\begin{table*}[t]
\centering
\resizebox{0.99\textwidth}{!}{
    \begin{tabular}{l||l||cc|cc|cc|cc|cc}
    \hline
     \makecell[c]{\multirow{2}{*}{Groups}}&\makecell[c]{\multirow{2}{*}{Methods}}& \multicolumn{2}{c|}{Depth Estimation} & \multicolumn{2}{c|}{Surface Normal} & \multicolumn{2}{c|}{Semantic Segmentation} & \multicolumn{2}{c|}{Keypoint Detection} & \multicolumn{2}{c}{Edge Detection}\\ \cline{3-12}
     &&Loss $\downarrow$&NormGain$_L$ (\%) $\uparrow$&Loss $\downarrow$&NormGain$_L$ (\%) $\uparrow$&Loss $\downarrow$&NormGain$_L$ (\%) $\uparrow$&Loss $\downarrow$&NormGain$_L$ (\%) $\uparrow$&Loss $\downarrow$&NormGain$_L$ (\%) $\uparrow$ \\ \hline
     &MTL&8.67e-3&-&	1.07e-1&-&	8.28e-2&-&	1.19e-2&-&	1.31e-2 \\
     &STL&1.60e-5&+99.82&	1.07e-1&-0.18&	9.16e-2&-10.63&	1.30e-4&+98.91&	1.56e-4&+98.81 \\ \hline
    \multirow{5}{*}{$K=3$} & RG      &2.57e-2& -195.88      &1.08e-1& -0.81    &8.43e-2& -1.88         &6.87e-3& +42.46        &6.88e-3& +47.45\\
                         & HOA    &5.85e-3& +32.47      &1.11e-1& -4.37   &7.33e-2& +11.49            &\textbf{2.00e-6}& \textbf{+99.98}        &8.60e-5& +99.34 \\
                         & TAG    &5.15e-3& +40.59      &1.21e-1& -12.93   &8.43e-2& -1.88          &\textbf{2.00e-6}& \textbf{+99.98}      &8.60e-5& +99.34\\
                         & MTG-Net &2.04e-4& +97.65      &\textbf{1.07e-1}& \textbf{+0.00}              &8.28e-2& +0.00                      &6.39e-4& +94.65        &4.08e-4& +96.88\\
                         & Ours    &\textbf{1.19e-7}& \textbf{+100.00}                &1.07e-1& -0.05   &\textbf{6.65e-2}& \textbf{+19.64}           &4.30e-5& +99.63        &\textbf{3.58e-7}& \textbf{+100.00}\\ \hline
    \multirow{5}{*}{$K=4$} & RG      &5.15e-3& +40.59         &1.07e-1& +0.00              &7.33e-2& +11.49              &1.19e-2& +0.00                  &6.88e-3& +47.45 \\
                         & HOA    &5.15e-3& +40.59         &1.06e-1& +0.44       &8.33e-2& -0.61              &\textbf{2.00e-6}& \textbf{+99.98}           &8.60e-5& +99.34\\
                         & TAG    &5.15e-3& +40.59         &1.11e-1& -4.37       &7.33e-2& +11.49              &\textbf{2.00e-6}& \textbf{+99.98}           &8.60e-5& +99.34\\
                         & MTG-Net &2.04e-4& +97.65         &1.07e-1& +0.00              &8.28e-2& +0.00                     &6.39e-4& +94.65           &4.08e-4& +96.88\\
                         & Ours    &\textbf{1.19e-7}& \textbf{+100.00}                &\textbf{1.05e-1}& \textbf{+1.43}       &\textbf{6.46e-2}& \textbf{+21.96}              &4.70e-5& +99.61          &\textbf{1.20e-5}& \textbf{+99.91}\\ \hline
    \multirow{5}{*}{$K=5$} & RG      &5.15e-3& +40.59         &1.07e-1& +0.00              &7.33e-2& +11.49              &6.87e-3& +42.46           &6.88e-3& +47.45\\
                         & HOA    &5.15e-3& +40.59         &1.06e-1& +0.44       &8.33e-2& -0.61              &2.00e-6& +99.98           &8.60e-5& +99.34\\
                         & TAG    &5.15e-3& +40.59         &1.11e-1& -4.37       &7.33e-2& +11.49              &2.00e-6& +99.98           &8.60e-5& +99.34\\
                         & MTG-Net &2.04e-4& +97.65         &1.07e-1& +0.00              &8.28e-2& +0.00                     &6.39e-4& +94.65           &4.08e-4& +96.88\\
                         & Ours    &\textbf{1.19e-7}& \textbf{+100.00}                &\textbf{1.05e-1}& \textbf{+1.62}       &\textbf{6.34e-2}& \textbf{+23.43}              &\textbf{1.00e-6}& \textbf{+99.99}           &\textbf{4.17e-7}& \textbf{+100.00}\\ \hline
    \end{tabular}}
    \caption{Performance on Taskonomy-5 \emph{w.r.t.} each input task. NormGain$_L$ is the normalized gain according to the task loss calculated by Eq. \eqref{eq:taskonomy error}, which is measured \emph{w.r.t.} Naive MTL.}
    \label{tab:taskonomy_per_task}
\end{table*}

\subsection{Experiments on Taskonomy with 5 Tasks}
Following \cite{hoa2020,tag2021,mtg2022}, we compare our methods with the state-of-the-art MTG methods including \textbf{HOA} \cite{hoa2020}, \textbf{TAG} \cite{tag2021}, and \textbf{MTG-Net} \cite{mtg2022}. 
% For HOA and TAG, we perform their codes on our GPU server. While for MTG-Net, we rely on the reported results from their paper \cite{mtg2022}, as MTG-Net requires to inefficiently sample numerous task combinations (up to $2^N$) and subsequent training them from scratch. 
We also report the performance of Random Group (\textbf{RG}) 
% which averages the performance of randomly dividing tasks into a given number of groups for XXX runs. 
which randomly divide the input tasks into a specific number of groups. 
We illustrate the baseline performance with \textbf{Naive MTL}, where all the tasks are trained simultaneously with a fully-shared encoder (\ie, within 1 group). We perform candidate numbers of groups as 3, 4, and 5.

The experimental results are shown in Table \ref{tab:taskonomy2}. Our method outperforms SOTA methods by a large margin with a more efficient $O(K)$ training complexity. Specifically, our approach has reduced the total loss by nearly $22\%$ compared to naive MTL and by $13\%$ compared to STL when $K=3$. As $K$ increases, our grouping performance further improves. Regarding the normalized metric NormGain \emph{w.r.t.} loss, \ie, Eq. \eqref{eq:taskonomy error}, it also achieves a remarkable improvement of over $60\%$ \emph{w.r.t.} naive MTL. 

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c||l||c|c||c}
\hline
 Groups&\makecell[c]{Methods}&Total Loss $\downarrow$& NormGain$_L$ (\%)  $\uparrow$&Relative Train. Complex. \\ \hline
 -&Naive MTL&0.223&-&$1$ \\
 -&STL&0.199&+57.35&$O(N)$ \\ \hline
 \multirow{5}{*}{$K=3$}&RG&0.231&-21.73&$O(K)$\\
 &HOA &0.190&+47.78&$O(N^2)+O(K)$\\
 &TAG &0.210&+45.02&$O(N)+O(K)$\\
 &MTG-Net &0.191&+57.83&$-$\\
 &Ours&\textbf{0.173}&\textbf{+63.85}&$O(K)$\\ \hline
 \multirow{5}{*}{$K=4$}&RG&0.204&+19.90&$O(K)$\\
 &HOA &0.195&+47.95&$O(N^2)+O(K)$\\
 &TAG &0.190&+49.41&$O(N)+O(K)$\\
 &MTG-Net &0.191&+57.83&$-$\\
 &Ours&\textbf{0.170}&\textbf{+64.58}&$O(K)$\\ \hline
 \multirow{5}{*}{$K=5$}&RG&0.198&+28.40&$O(K)$\\
 &HOA &0.195&+47.95&$O(N^2)+O(K)$\\
 &TAG &0.190&+49.41&$O(N)+O(K)$\\
 &MTG-Net &0.191&+57.83&$-$\\
 &Ours&\textbf{0.168}&\textbf{+65.01}&$O(K)$\\ \hline
\end{tabular}}
\caption{Experimental results on Taskonomy-5. NormGain$_L$ is the normalized gain according to the task loss calculated by Eq. \eqref{eq:taskonomy error}. NormGain$_L$ and relative training complexity are measured \emph{w.r.t.} Naive MTL.}
\label{tab:taskonomy2}
\end{table}

It can be observed that the performances in terms of total loss and NormGain are not consistent for some MTG methods, which perform well in total loss but degrade in NormGain. This is because, as discussed in Sect. \ref{sec:metrics}, the total loss is affected by loss magnitudes associated with different tasks, a slight improvement in a task with a large loss magnitude might overshadow a significant degradation in a task with a small loss magnitude. In contrast, our proposed NormGain addresses this issue by eliminating such undesirable influence through normalization, providing a better measure of the improvement on all the tasks. We validate this by illustrating the loss and the relative gain \emph{w.r.t.} Naive MTL \emph{for each task} in Table \ref{tab:taskonomy_per_task}, where our method achieves the best performance across almost all tasks.

We also show the training complexity relative to the Naive MTL method in Table \ref{tab:taskonomy_per_task}. Given $K << N$, Our method achieves the best training efficiency except for Naive MTL which simply shares the whole encoder and cannot deliver desirable accuracy. Note that there are two terms for the training complexity of HOA and TAG, as they involve first identifying task groups according to $N$ tasks, then training $K$ networks, each for a task group, from scratch. The training complexity of MTG-Net is not included as it requires up to $O(2^N)+O(K)$ to sample up to $2^N$ task combinations and subsequent training them from scratch\footnote{For the Taskonomy-5 experiment, MTG-Net samples 31 task combinations with 5 input tasks, as reported in \cite{mtg2022}, resulting in a complexity of $O(2^N)+O(K)$.}.  % We illustrate the training time of each method in Fig. \ref{img:running time}.


% Except for RG, the training complexity of other grouping methods all is related to task numbers. For them, finding the best group on only $5$ tasks has consumed hundreds of thousands of Tesla V100 GPU hours \cite{tag2021}, excluding the training time for models on the identified group. It is inconceivable to group tasks on a larger scale circumstance, \eg, autonomous driving that need dozens of vision tasks to be cooperative. 



\begin{table}[t]
\centering
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{c||l||c|c||c}
\hline
 Groups&\makecell[c]{Methods}&Total Error $\downarrow$&NormGain$_E$ (\%) $\uparrow$&Relative Train. Complex. \\ \hline
 -&Naive MTL&56.13&-& 1 \\
 -&STL&59.93&-8.70&$O(N)$ \\ \hline
 % -&GradNorm &-0.20&$O(N)$ \\
 % -&PCGrad &+0.02&$O(N)$ \\ \hline
 \multirow{4}{*}[-0.5ex]{$K=2$}
 &RG&54.87&+1.06&$O(K)$ \\
 &HOA &53.60&+3.27&$O(N^2) + O(K)$ \\
 &TAG &53.41&+4.38&$O(N) + O(K)$ \\
 &Ours&\textbf{52.97}&\textbf{+5.75}&$O(K)$ \\ 
 \hline
 \multirow{4}{*}[-0.5ex]{$K=3$}
 &RG&54.57&+1.54&$O(K)$ \\
 &HOA &54.04&+3.62&$O(N^2) + O(K)$ \\
 &TAG &54.37&+2.08&$O(N) + O(K)$ \\
 &Ours&\textbf{53.67}&\textbf{+4.64}&$O(K)$ \\ 
 \hline
 \multirow{4}{*}[-0.5ex]{$K=4$}
 &RG&54.57&+1.54&$O(K)$ \\
 &HOA &54.14&+2.53&$O(N^2) + O(K)$ \\
 &TAG &54.11&+3.17&$O(N) + O(K)$ \\
 &Ours&\textbf{53.62}&\textbf{+4.62}&$O(K)$ \\ 
 \hline
\end{tabular}}
\caption{Experimental results on CelebA-9. As all the input tasks are classifications, we report the total classification error and NormGain$_E$, \ie, the normalized gain according to the task loss calculated by Eq. \eqref{eq:classification error}. NormGain$_E$ and relative training complexity are measured in terms of Naive MTL.}
\label{tab:celeba}
\end{table}



% Figure \ref{mtl radar} displays three radar plots concerning the improvement of grouping methods on each task relative to naive MTL, for $K=3, 4, 5$. It shows that our impressive performance benefits from comprehensive improvements across all tasks, stronger than most of comparative methods. On the semantic segmentation task, the proposed approach is beyond all other methods, particularly at $K=5$. The visualization relative to STL is presented in the appendix \ref{subsec: relative to stl}.

\subsection{Experiments on CelebA with 9 Tasks}

We compare our method with the state-of-the-art methods \textbf{HOA} \cite{hoa2020} and \textbf{TAG} \cite{tag2021}. MTG-Net \cite{mtg2022} is not included in CelebA-9 as MTG-Net requires to inefficiently sample up to $2^N$ task combinations and subsequent training them from scratch, which takes \emph{thousands of GPU hours} as reported in \cite{mtg2022}.
% We also take MTO methods into account, which project gradients from different tasks, including \textbf{GradNorm} \cite{gradnorm12018}, and \textbf{PCGrad} \cite{yugradient2020}. 
Following \cite{tag2021}, we perform candidate numbers of groups as 2, 3, and 4 on CelebA-9. As all the input tasks in this experiment are classification tasks, therefore we report the total classification error and NormGain \emph{w.r.t.} classification error, \ie, Eq. \eqref{eq:classification error}, in Table \ref{tab:celeba}. Table \ref{tab:celeba} illustrates the experiments results on CelebA-9, showing that
% , where the results from the state-of-the-art methods are derived from \cite{tag2021} and Eq. \eqref{eq:classification error}.  
our method consistently outperforms the state-of-the-art methods on the CelebA-9 experiments by a large margin with least training complexity of $O(K)$.

% In addition, almost all the MTG methods surpass MTO methods in Table \ref{tab:celeba experiments}, suggesting that it may not be sufficient to improve MTL solely by gradient manipulations.








% \begin{figure*}[t]
%     \vspace{4mm}
%     \centering
%     \includegraphics[width=0.85\textwidth]{image/taskonomy_bar_mtl.pdf}
%     \caption{Relative improvement of grouping methods in terms of Naive MTL for each task on the Taskonomy dataset with 5 tasks over 3, 4, and 5 groups. The value of relative improvement lower than $-0.2$ has been truncated here.}
%     \label{mtl radar}
%     \vspace{2mm}
% \end{figure*}

% \begin{figure*}[t]


\section{Ablation Analysis}
It is interesting to validate i) whether our proposed one-shot MTG outperforms the existing two-phase methods \cite{hoa2020,tag2021,mtg2022} given the same group categorization, ii) can our method generalize to transformer backbone, iii) can our method scale to more input tasks, and iv) what is the influence if we share more or less encoder layers in our method. We carefully investigate those issues in this section.


% In this section, we perform extensive ablation analysis regarding the merit of the proposed one-shot nature for MTG, the generalizing-ability of our method to transformer backbone, the scalability of our method to a large number of input tasks, and the flexibility of our method with different amounts of shared backbone layers.

\subsection{Merits of One-shot Nature for MTG} 

The one-shot simultaneous group identification and grouped task learning is one of the key features of our method. Benefit from that, our method is able to i) avoid the potential objective bias in the existing two-phase methods \cite{hoa2020,tag2021,mtg2022}, where group identification and grouped task learning act as separated sequential procedures, and ii) further accelerate the training procedure as retraining from scratch is no longer needed. In order to better validate them, we perform ablation using the group categorizations discovered by our method, and retrain them from \emph{scratch} and from \emph{Naive MTL initialization}. As shown in Table \ref{tab:taskonomy_retrain}, our one-shot method significantly outperforms its both counterparts with the same group categorization.

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c||l||c|c}
\hline
 Groups&\makecell[c]{Methods}&Total Loss $\downarrow$&NormGain$_L$ (\%) $\uparrow$ \\ \hline
 \multirow{3}{*}{$K=3$}&Retrain from Scratch&0.183&+53.34 \\
 &Retrain from Naive MTL Init.&0.194&+57.10 \\
 &Ours&\textbf{0.173}&\textbf{+63.85} \\ \hline
 \multirow{3}{*}{$K=4$}&Retrain from Scratch&0.183&+53.34 \\
 &Retrain from Naive MTL Init.&0.194&+57.10 \\
 &Ours&\textbf{0.170}&\textbf{+64.58} \\ \hline
 \multirow{3}{*}{$K=5$}&Retrain from Scratch&0.190&+59.47 \\
 &Retrain from Naive MTL Init.&0.194&+58.87 \\
 &Ours&\textbf{0.168}&\textbf{+65.01} \\ \hline
\end{tabular}}
\caption{Ablation on the merits of one-shot nature for MTG. We use the same group categorization for all the methods. We perform two double-shot MTG methods, which are retrained from \emph{scratch} and \emph{Naive MTL initialization}, respectively.}
\label{tab:taskonomy_retrain}
\end{table}

\subsection{Generalizing-ability to Transformer Backbone} 

We re-perform the Taskonomy-5 experiment by replacing the variant of Xception by ViTBase \cite{dosovitskiy2020image}. The results are shown in Table XXX, illustrating a consistent improvement over Naive MTL using different backbones.


\subsection{Scalability to More Input Tasks} 

We validate our method with a more challenging case of categorizing \textbf{40} tasks into 5 groups on the CelebA dataset. We illustrate the relative gain \emph{w.r.t.} Naive MTL method for each task in Fig. \ref{img:celeba-40}. Figure \ref{img:celeba-40} shows that, in most cases, our method reduces the task loss by categorizing and optimizing collaborative tasks within the same group, particularly on tasks of \textit{Wearing\_Lipstick} and \textit{Pointy\_nose}. % The poor performance on \textit{Chubby} is attributed to its ambiguous definition, prompting the need for more training tasks to constrain the model.


\subsection{Flexibility with Different Amounts of Shared Backbone Layers}

As shown in Fig. \ref{img:framework}, our method enables to share the backbone encoder layers across different groups, which introduce a flexible design regarding a further training efficiency (\ie, sharing more layers) and a better representation capability (\ie, sharing less layers). We perform ablations with 0, 6, 9 shared layers in Table \ref{tab:shared and no shared}, which demonstrates XXX.

\begin{table}[t]
\centering
\resizebox{0.92\columnwidth}{!}{
\begin{tabular}{c|ccc}
\hline
Shared layers & Total loss $\downarrow$  & $\text{NormGain}_{L}$ (\%) $\uparrow$ & FLOPs (G) \\ \hline
0             & 0.174 & 63.72         & 28.45     \\
6             & 0.173 & 63.85         & 21.33     \\ 
9             & 0.169 & 64.75         & 16.68    \\ \hline
\end{tabular}}
\caption{}
\label{tab:shared and no shared}
\end{table}

% In this section, we investigate the impact of incorporating the optional shared layers across groups. The average relative improvement results according to Naive MTL on CelebA-9 are presented in Table \ref{tab:shared and no shared}. Table \ref{tab:shared and no shared} indicates that the performance without shared layers across groups is comparable to that with shared layers, while the latter is able to achieve additional efficiency improvements. 

% \begin{table}[t]
% \small
% \centering
% \caption{Ablation analysis about with and without the optional shared backbone. The first two columns are the average relative improvement $\text{ARI}_{cls}$ according to the Naive MTL, which indicates the comparable performance of both options. The last column indicates the ratios of the FLOPs for configurations with a shared backbone divided by those without a shared backbone.}
% \vspace{1mm}
% \begin{tabular}{c|c|c|c}
% \hline
% \multirow{2}{*}{Groups}&\multicolumn{2}{c|}{Performance ($\text{ARI}_{cls}$)}&Efficiency \\ \cline{2-4}
% &w/ shared&w/o shared&FLOPs ratio (\%) \\ \hline
% $K=2$&3.84&5.17&94.90 \\
% $K=3$&4.01&4.51&93.21 \\
% $K=4$&3.40&0.16&92.36 \\ \hline
% \end{tabular}
% \label{tab:shared and no shared}
% \vspace{-5mm}
% \end{table}





==> sec/5_conclusion.tex <==
\section{Conclusion}

In this paper, we tackle the challenges of Multi-Task Learning with numerous tasks using Multi-Task Grouping techniques. Our approach efficiently identifies the best task groups from $2^N$ candidates for the input $N$ tasks, with the high-order task affinity fully exploited. Moreover, our unified training approach to group identification and grouped task learning can be directly optimized using the task losses in one shot, which further improves the training efficiency and mitigates potential bias in separate training. We efficiently implement our method as a pruning problem, where the pruning process is also efficient as only the task heads are expended to prune rather than the task-specific encoders. We validate our methods on both CelebA and Taskonomy datasets, by categorizing 5, 9, and 40 tasks into various groups. The results demonstrate the promising performance and the desirable efficiency of our method.
